Subquantum Pilot-Wave System Theory: Structural and Amplitude Nonequilibrium under Source Fields

A source in the Schrodinger equation changes the norm of the guiding wave, apparently conflicting with the conservation of probability. In source-extended de Broglie-Bohm dynamics the conflict disappears: probability is carried by the particle ensemble, while the wavefunction guides its motion. The difficulty is then different. What does quantum equilibrium mean when the particle distribution remains normalized but the guiding density does not? We show that the departure has two independent components: a structural one, measured by the Kullback--Leibler divergence between the particle distribution and the normalized guiding density, and an amplitude one, measured by the Born weight. The Born rule holds precisely when both are equilibrated. Their evolution is governed by the complex source-to-wavefunction ratio; scale covariance further distinguishes an independently prescribed source, against which the amplitude of the wave matters, from state-dependent generators for which rescaling remains a symmetry. We develop a source-aware analytical--computational method, combining exact or semi-analytical guiding fields with Bohmian trajectory transport, ensemble quadrature and independent numerical checks. Free-space impulses expose the limits of global diagnostics and an exact jump rule; a driven ring has constant Born weight but either periodic or secular structural departure; oscillators show both source-generated structural change and amplitude-only evolution, including a finite-horizon weak-drive plateau far below its frozen-particle value; and a coupled two-body model exhibits nonlocal guidance and evolving particle entanglement. The source-free, initially equilibrated sector recovers standard quantum mechanics.

==> numbers.tex <==
%% generated by code/make_numbers.py -- do not edit
\makeatletter
\expandafter\def\csname nv@DADB\endcsname{2.6\!\times\!10^{-13}}
\expandafter\def\csname nv@DEightAdapt\endcsname{0.19908}
\expandafter\def\csname nv@DEightUni\endcsname{0.19910}
\expandafter\def\csname nv@KLfrozen\endcsname{1.2704}
\expandafter\def\csname nv@KLfrozenQ\endcsname{1.2700}
\expandafter\def\csname nv@NBquad\endcsname{2.2\!\times\!10^{-14}}
\expandafter\def\csname nv@adaptNodes\endcsname{2827}
\expandafter\def\csname nv@avgDtrue\endcsname{0.244}
\expandafter\def\csname nv@avgErrNB\endcsname{0.244}
\expandafter\def\csname nv@avgNBtrue\endcsname{4.047}
\expandafter\def\csname nv@avgNBwrong\endcsname{3.803}
\expandafter\def\csname nv@crossJ\endcsname{0.2}
\expandafter\def\csname nv@crossJscan\endcsname{4.4, 4.2, 1.3}
\expandafter\def\csname nv@crossMax\endcsname{5.4}
\expandafter\def\csname nv@crossMin\endcsname{3.0}
\expandafter\def\csname nv@crossTPAt3\endcsname{6753}
\expandafter\def\csname nv@crossV1At3\endcsname{150}
\expandafter\def\csname nv@hoDA\endcsname{0.619}
\expandafter\def\csname nv@hoDB\endcsname{0.371}
\expandafter\def\csname nv@hoDC\endcsname{0.244}
\expandafter\def\csname nv@hoDD\endcsname{0.120}
\expandafter\def\csname nv@hoDipA\endcsname{4.9\!\times\!10^{-4}}
\expandafter\def\csname nv@hoDipB\endcsname{9.0\!\times\!10^{-4}}
\expandafter\def\csname nv@hoDipC\endcsname{1.6\!\times\!10^{-3}}
\expandafter\def\csname nv@hoDipD\endcsname{1.6\!\times\!10^{-3}}
\expandafter\def\csname nv@hoDmaxA\endcsname{0.622}
\expandafter\def\csname nv@hoDmaxB\endcsname{0.372}
\expandafter\def\csname nv@hoDmaxC\endcsname{0.245}
\expandafter\def\csname nv@hoDmaxD\endcsname{0.120}
\expandafter\def\csname nv@hoFourA125\endcsname{0.227}
\expandafter\def\csname nv@hoFourA250\endcsname{0.245}
\expandafter\def\csname nv@hoFourA500\endcsname{0.253}
\expandafter\def\csname nv@hoFourB125\endcsname{0.104}
\expandafter\def\csname nv@hoFourB250\endcsname{0.167}
\expandafter\def\csname nv@hoFourB500\endcsname{0.203}
\expandafter\def\csname nv@hoFourC125\endcsname{0.048}
\expandafter\def\csname nv@hoFourC250\endcsname{0.120}
\expandafter\def\csname nv@hoFourC500\endcsname{0.180}
\expandafter\def\csname nv@hoFourDmaxRescale\endcsname{0.20}
\expandafter\def\csname nv@hoFourEndA\endcsname{0.2572}
\expandafter\def\csname nv@hoFourEndB\endcsname{0.2243}
\expandafter\def\csname nv@hoFourEndC\endcsname{0.2236}
\expandafter\def\csname nv@hoFourOrd\endcsname{yes}
\expandafter\def\csname nv@hoFourRescale\endcsname{1.2\!\times\!10^{-12}}
\expandafter\def\csname nv@hoFourT\endcsname{600}
\expandafter\def\csname nv@hoQA\endcsname{4.9\!\times\!10^{-4}}
\expandafter\def\csname nv@hoQB\endcsname{3.1\!\times\!10^{-4}}
\expandafter\def\csname nv@hoQC\endcsname{1.2\!\times\!10^{-4}}
\expandafter\def\csname nv@hoQD\endcsname{1.7\!\times\!10^{-4}}
\expandafter\def\csname nv@hoStepsA\endcsname{2478}
\expandafter\def\csname nv@hoStepsB\endcsname{2157}
\expandafter\def\csname nv@hoStepsC\endcsname{1985}
\expandafter\def\csname nv@hoStepsD\endcsname{1629}
\expandafter\def\csname nv@hoThreeEnd0\endcsname{0.223}
\expandafter\def\csname nv@hoThreeEnd0p5\endcsname{0.268}
\expandafter\def\csname nv@hoThreeEnd1\endcsname{0.180}
\expandafter\def\csname nv@hoThreeEnd1p5\endcsname{0.051}
\expandafter\def\csname nv@hoThreeEnd2\endcsname{0.022}
\expandafter\def\csname nv@hoThreeMax0\endcsname{0.223}
\expandafter\def\csname nv@hoThreeMax0p5\endcsname{0.268}
\expandafter\def\csname nv@hoThreeMax1\endcsname{0.180}
\expandafter\def\csname nv@hoThreeMax1p5\endcsname{0.071}
\expandafter\def\csname nv@hoThreeMax2\endcsname{0.077}
\expandafter\def\csname nv@hoThreeNB0\endcsname{8.1\!\times\!10^{-14}}
\expandafter\def\csname nv@hoThreeNB0p5\endcsname{8.1\!\times\!10^{-14}}
\expandafter\def\csname nv@hoThreeNB1\endcsname{8.1\!\times\!10^{-14}}
\expandafter\def\csname nv@hoThreeNB1p5\endcsname{8.1\!\times\!10^{-14}}
\expandafter\def\csname nv@hoThreeNB2\endcsname{8.1\!\times\!10^{-14}}
\expandafter\def\csname nv@hoThreeT020\endcsname{20}
\expandafter\def\csname nv@hoThreeT020p5\endcsname{14}
\expandafter\def\csname nv@hoThreeT021\endcsname{8}
\expandafter\def\csname nv@hoThreeT021p5\endcsname{10}
\expandafter\def\csname nv@hoThreeT022\endcsname{8}
\expandafter\def\csname nv@hoThreeTmax0\endcsname{600}
\expandafter\def\csname nv@hoThreeTmax0p5\endcsname{600}
\expandafter\def\csname nv@hoThreeTmax1\endcsname{600}
\expandafter\def\csname nv@hoThreeTmax1p5\endcsname{30}
\expandafter\def\csname nv@hoThreeTmax2\endcsname{24}
\expandafter\def\csname nv@hoTwoD\endcsname{2.2\!\times\!10^{-14}}
\expandafter\def\csname nv@hoTwoGam\endcsname{3.3\!\times\!10^{-16}}
\expandafter\def\csname nv@hoTwoNB\endcsname{2.2\!\times\!10^{-14}}
\expandafter\def\csname nv@hoTwoShift\endcsname{2.7\!\times\!10^{-14}}
\expandafter\def\csname nv@identDev\endcsname{2.9\!\times\!10^{-11}}
\expandafter\def\csname nv@jumpDADB\endcsname{3.3\!\times\!10^{-9}}
\expandafter\def\csname nv@jumpDirect0p025\endcsname{0.1460}
\expandafter\def\csname nv@jumpDirect0p05\endcsname{0.1470}
\expandafter\def\csname nv@jumpDirect0p1\endcsname{0.1488}
\expandafter\def\csname nv@jumpDirect0p2\endcsname{0.1515}
\expandafter\def\csname nv@jumpDjump\endcsname{0.1450}
\expandafter\def\csname nv@jumpDno\endcsname{0.4231}
\expandafter\def\csname nv@jumpHi\endcsname{0.28}
\expandafter\def\csname nv@jumpLo\endcsname{-1.31}
\expandafter\def\csname nv@jumpNB\endcsname{1.5267}
\expandafter\def\csname nv@jumpPW0\endcsname{1.8\!\times\!10^{-2}}
\expandafter\def\csname nv@jumpPW4\endcsname{1.7\!\times\!10^{-3}}
\expandafter\def\csname nv@jumpPWeps0\endcsname{0.04}
\expandafter\def\csname nv@jumpPWeps4\endcsname{0.0025}
\expandafter\def\csname nv@jumpPred\endcsname{0.1450}
\expandafter\def\csname nv@jumpScale\endcsname{1.21}
\expandafter\def\csname nv@ladD0\endcsname{8.1\!\times\!10^{-7}}
\expandafter\def\csname nv@ladD1\endcsname{3.8\!\times\!10^{-9}}
\expandafter\def\csname nv@ladD2\endcsname{1.2\!\times\!10^{-11}}
\expandafter\def\csname nv@ladQ0\endcsname{5.2\!\times\!10^{-6}}
\expandafter\def\csname nv@ladQ1\endcsname{4.0\!\times\!10^{-8}}
\expandafter\def\csname nv@ladQ2\endcsname{3.3\!\times\!10^{-10}}
\expandafter\def\csname nv@ladSteps0\endcsname{384}
\expandafter\def\csname nv@ladSteps1\endcsname{454}
\expandafter\def\csname nv@ladSteps2\endcsname{736}
\expandafter\def\csname nv@ladTol0\endcsname{1\!\times\!10^{-6}}
\expandafter\def\csname nv@ladTol1\endcsname{1\!\times\!10^{-8}}
\expandafter\def\csname nv@ladTol2\endcsname{1\!\times\!10^{-10}}
\expandafter\def\csname nv@leadErrSmall\endcsname{0.7}
\expandafter\def\csname nv@leadErrSmallMin\endcsname{0.3}
\expandafter\def\csname nv@leadOrd\endcsname{2.0}
\expandafter\def\csname nv@pdeCoh\endcsname{1.0\!\times\!10^{-10}}
\expandafter\def\csname nv@pdeHO\endcsname{4.3\!\times\!10^{-13}}
\expandafter\def\csname nv@pdeMax\endcsname{1.8\!\times\!10^{-10}}
\expandafter\def\csname nv@pdePulse\endcsname{1.8\!\times\!10^{-10}}
\expandafter\def\csname nv@pdeRing\endcsname{1.4\!\times\!10^{-13}}
\expandafter\def\csname nv@pdeTwo\endcsname{2.6\!\times\!10^{-12}}
\expandafter\def\csname nv@quadSpread\endcsname{1.4\!\times\!10^{-5}}
\expandafter\def\csname nv@rateD\endcsname{1.1\!\times\!10^{-4}}
\expandafter\def\csname nv@rateNB\endcsname{1.6\!\times\!10^{-9}}
\expandafter\def\csname nv@ringDADBu\endcsname{7.9\!\times\!10^{-11}}
\expandafter\def\csname nv@ringDendT\endcsname{18.60}
\expandafter\def\csname nv@ringDmax\endcsname{0.2231}
\expandafter\def\csname nv@ringDmin\endcsname{0.1148}
\expandafter\def\csname nv@ringDper\endcsname{5.2\!\times\!10^{-11}}
\expandafter\def\csname nv@ringDslope\endcsname{0.6455}
\expandafter\def\csname nv@ringDzero\endcsname{0.2231}
\expandafter\def\csname nv@ringDzeroErr\endcsname{1.1\!\times\!10^{-16}}
\expandafter\def\csname nv@ringFracAtt\endcsname{99.8}
\expandafter\def\csname nv@ringFracBig\endcsname{72}
\expandafter\def\csname nv@ringInvT\endcsname{6.1\!\times\!10^{-6}}
\expandafter\def\csname nv@ringInvTbig\endcsname{1.4\!\times\!10^{-5}}
\expandafter\def\csname nv@ringInvU\endcsname{5.5\!\times\!10^{-11}}
\expandafter\def\csname nv@ringLamClosed\endcsname{0.645497}
\expandafter\def\csname nv@ringLamFit\endcsname{0.645497}
\expandafter\def\csname nv@ringLamSpread\endcsname{1.4\!\times\!10^{-4}}
\expandafter\def\csname nv@ringNBdev\endcsname{2.2\!\times\!10^{-16}}
\expandafter\def\csname nv@ringPhase\endcsname{2.6\!\times\!10^{-11}}
\expandafter\def\csname nv@ringStepsU\endcsname{2712}
\expandafter\def\csname nv@ringT\endcsname{3.68406}
\expandafter\def\csname nv@ringTend\endcsname{30}
\expandafter\def\csname nv@ringTquad\endcsname{3.68406}
\expandafter\def\csname nv@ringVmax\endcsname{0.667}
\expandafter\def\csname nv@ringVmin\endcsname{-2.000}
\expandafter\def\csname nv@scipyF\endcsname{5.6\!\times\!10^{-13}}
\expandafter\def\csname nv@scipyQ\endcsname{1.0\!\times\!10^{-13}}
\expandafter\def\csname nv@spCohA\endcsname{1.4\!\times\!10^{-5}}
\expandafter\def\csname nv@spCohC\endcsname{8.8\!\times\!10^{-7}}
\expandafter\def\csname nv@spCohOrd\endcsname{2.0}
\expandafter\def\csname nv@spHOA\endcsname{3.7\!\times\!10^{-6}}
\expandafter\def\csname nv@spHOC\endcsname{2.3\!\times\!10^{-7}}
\expandafter\def\csname nv@spHOOrd\endcsname{2.0}
\expandafter\def\csname nv@spPulseA\endcsname{4.6\!\times\!10^{-14}}
\expandafter\def\csname nv@spPulseC\endcsname{1.9\!\times\!10^{-13}}
\expandafter\def\csname nv@spPulseOrd\endcsname{-1.1}
\expandafter\def\csname nv@spRingA\endcsname{3.4\!\times\!10^{-7}}
\expandafter\def\csname nv@spRingC\endcsname{2.1\!\times\!10^{-8}}
\expandafter\def\csname nv@spRingOrd\endcsname{2.0}
\expandafter\def\csname nv@spTwoA\endcsname{2.4\!\times\!10^{-5}}
\expandafter\def\csname nv@spTwoC\endcsname{1.5\!\times\!10^{-6}}
\expandafter\def\csname nv@spTwoOrd\endcsname{2.0}
\expandafter\def\csname nv@twoDADB\endcsname{6.5\!\times\!10^{-10}}
\expandafter\def\csname nv@twoDend\endcsname{0.162}
\expandafter\def\csname nv@twoDiff1d\endcsname{2.5\!\times\!10^{-3}}
\expandafter\def\csname nv@twoDiffCoarse\endcsname{1.2\!\times\!10^{-2}}
\expandafter\def\csname nv@twoDmax\endcsname{0.187}
\expandafter\def\csname nv@twoJ\endcsname{0.3}
\expandafter\def\csname nv@twoNB\endcsname{7.2\!\times\!10^{-15}}
\expandafter\def\csname nv@twoNtraj\endcsname{5329}
\expandafter\def\csname nv@twoPtF\endcsname{4.3\!\times\!10^{-9}}
\expandafter\def\csname nv@twoPtQ\endcsname{4.8\!\times\!10^{-9}}
\expandafter\def\csname nv@twoPtX\endcsname{1.4\!\times\!10^{-14}}
\expandafter\def\csname nv@twoTend\endcsname{10}
\expandafter\def\csname nv@twoVCM\endcsname{4.4\!\times\!10^{-16}}
\expandafter\def\csname nv@twoVhi\endcsname{3.60}
\expandafter\def\csname nv@twoVlo\endcsname{0.02}
\expandafter\def\csname nv@twoW\endcsname{1.4142}
\expandafter\def\csname nv@weakD100A\endcsname{0.2286}
\expandafter\def\csname nv@weakD100B\endcsname{0.2240}
\expandafter\def\csname nv@weakD100C\endcsname{0.2247}
\expandafter\def\csname nv@weakD100D\endcsname{0.2251}
\expandafter\def\csname nv@weakDA\endcsname{0.2288}
\expandafter\def\csname nv@weakDB\endcsname{0.2242}
\expandafter\def\csname nv@weakDC\endcsname{0.2249}
\expandafter\def\csname nv@weakDD\endcsname{0.2251}
\expandafter\def\csname nv@weakDeltaA\endcsname{1.7\!\times\!10^{-4}}
\expandafter\def\csname nv@weakDeltaB\endcsname{1.6\!\times\!10^{-4}}
\expandafter\def\csname nv@weakDeltaC\endcsname{1.7\!\times\!10^{-4}}
\expandafter\def\csname nv@weakDeltaD\endcsname{0}
\expandafter\def\csname nv@weakExtrap\endcsname{0.225}
\expandafter\def\csname nv@weakMax\endcsname{0.229}
\expandafter\def\csname nv@weakMin\endcsname{0.224}
\expandafter\def\csname nv@weakN\endcsname{4}
\expandafter\def\csname nv@weakQuadA\endcsname{3.2\!\times\!10^{-5}}
\expandafter\def\csname nv@weakQuadB\endcsname{2.0\!\times\!10^{-4}}
\expandafter\def\csname nv@weakStepsA\endcsname{65944}
\expandafter\def\csname nv@weakStepsB\endcsname{130017}
\expandafter\def\csname nv@weakStepsC\endcsname{260122}
\expandafter\def\csname nv@weakStepsD\endcsname{244421}
\expandafter\def\csname nv@weakTendA\endcsname{1000}
\expandafter\def\csname nv@weakTendB\endcsname{2000}
\expandafter\def\csname nv@weakTendC\endcsname{4000}
\expandafter\def\csname nv@weakTendD\endcsname{4000}
\makeatother
\newcommand{\nv}[1]{\ensuremath{\csname nv@#1\endcsname}}

